PriMock57: A Dataset Of Primary Care Mock Consultations

Recent advances in Automatic Speech Recognition (ASR) have made it possible to reliably produce automatic transcripts of clinician-patient conversations. However, access to clinical datasets is heavily restricted due to patient privacy, thus slowing down normal research practices. We detail the development of a public access, high quality dataset comprising of57 mocked primary care consultations, including audio recordings, their manual utterance-level transcriptions, and the associated consultation notes. Our work illustrates how the dataset can be used as a benchmark for conversational medical ASR as well as consultation note generation from transcripts.

==> sections/L_ie.tex <==
\section{Clinical information extraction evaluation} \label{sec:information-extraction}
\begin{itemize}
    \item Stanza + fuzzly
    \item Amazon Comprehend Medical
    \item John Snow
    \item Medcat
    \item Azure NLP
    \item Babylon stuff
\end{itemize}

Temporary results table in Figure \ref{fig:ie-results}.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/ie-results.png}
    \caption{Information Extraction engine comparison. (This image is temporary, we should replace it with a table - some of the information should be dropped.)}
    \label{fig:ie-results}
\end{figure*}

% USE THIS WHEN TALKING ABOUT POOLING
%The i2b2 clinical NER annotation schema is fairly established within the academic community but as companies are building clinical information extraction products this standard is not always used. For example, Amazon Comprehend Medical (ACM) considers medication to be a separate category, while i2b2 considers them a part of treatments, and vice versa, ACM groups tests with treatments while i2b2 keeps them in separate categories. Instead of choosing one of the approaches, we thought it would be more pragmatical to design a more coarse scheme with a single category to replace the Tests and Treatments categories in the i2b2 scheme
